DuSK: Faster Indirect Text Entry Supporting Out-Of-Vocabulary Words for Touchpads

Given the ubiquity of SmartTVs and head-mounted-display-based virtual environments, recent research has explored techniques to support eyes-free text entry using touchscreen devices. However, proposed techniques, leveraging lexicons, limit the user's ability to enter out-of-vocabulary words. In this paper, we investigate how to enter text while relying on unambiguous input to support out-of-vocabulary words. Through an iterative design approach, and after a careful investigation of actions that can be accurately and rapidly performed eyes-free, we devise DuSK, a {Du}al-handed, {S}troke-based, 1{K}eyboarding technique. In a controlled experiment, we show initial speeds of 10 WPM steadily increasing to 13~WPM with training. DuSK outperforms the common cursor-based text entry technique widely deployed in commercial SmartTVs (8 WPM) and is comparable to other eyes-free lexicon-based techniques, but with the added benefit of supporting out-of-vocabulary word input.

==> tex/CHI_reviews.tex <==
1AC review
score 3/5

  Expertise

    Knowledgeable

  Recommendation

    Neutral: I am unable to argue for accepting or rejecting this paper; 3.0

  1AC: The Meta-Review

    The reviewers have many compliments for this paper, calling it "well-executed"
    (R3), "insightful" (R3), and "clear" (R1). R3 appreciates that the sequence of
    user studies and the explanation of the iterative design process provided many
    insights. R1 and I also appreciate the fact that the authors plan on open-sourcing
    their codebase with their paper, which will enable other researchers to build off
    of DuSK or compare their own systems to it.

    In my meta-review, I have done my best to summarize the concerns raised by the
    reviewers; however, I encourage the authors to read each of the reviews in detail
    for any smaller suggestions that may not be captured in my summary. Although the
    reviewer scores are generally neutral, multiple reviewers note that they are
    looking forward to a strong rebuttal that will address their concerns so that they
    can give positive scores. For the sake of staying within the range of scores given
    by the other reviewers, I will give a neutral score as well. However, I am leaning
    in favor of accepting this paper pending that the issues listed in this meta-
    review are sufficiently addressed.

    MOTIVATION AND SUPPORT OF DUSK'S DESIGN GOALS (R1, R3)
    R3 wants to see more motivation for DuSK's design goals. The authors mention that
    eyes-free text entry would be useful for SmartTVs and VR applications, but the
    requirement of an extra device (i.e., a smartphone) makes such applications less
    attractive. One of the most commonly referenced goals in the paper is that DuSK
    should be able to support OOV words. However, R3 does not find the motivation for
    this goal to be very strong. Furthermore, R1 and R2 question whether DuSK's
    ability to support OOV words was sufficiently tested since the MacKenzie-Soukoreff
    phrase set does not include many OOV words, and auto-correction can influence
    people's behavior when typing OOV words.

    DESIGN RATIONALE (R1, R2)
    Although the reviewers appreciate the methodical nature of the sequential studies
    and the iterative design process, many of the reviewers have questions about how
    Study 1 was used to inform the design of DuSK and the future studies. R2 comments
    that taps were the fastest and most accurate gestures in Study 1, yet taps were
    only used to select the starting positions ('D' and 'K'). R1 notes that users were
    able to benefit from visual feedback in the final design of DuSK, but such
    feedback was not available in Study 1. Stroke and tap gestures benefit more from
    visual cursor feedback than gestural inputs, which could explain why the L- and
    V-shape strokes were abandoned early on. Also, R1 wants an explanation for why the
    'D' and 'K' keys were selected as the starting points for input gestures.

    VALIDITY OF THE EXPERT EVALUATION (R1)
    Some concerns are raised about the final evaluation that compared the expert and
    novel DuSK users. R1 questions whether having the authors as expert users provided
    an unfair advantage to them since they "know all the tricks of the technique".
    Because the experts were authors, they may have had experience with DuSK before
    being officially evaluated in that study. Along those lines, we would like to see
    more information about the experts' learning curves.

    PRIOR WORK (R1)
    R1 lists additional prior work that the reviewers may want to consider adding to
    their own literature review.

  Rebuttal response

    (blank)

----------------------------------------------------------------

2AC review
score 3/5

  Expertise

    Knowledgeable

  Recommendation

    Neutral: I am unable to argue for accepting or rejecting this paper; 3.0

  Review

    In this paper, the authors present DuSK an indirect text entry method for
    touchpads. Since DuSK does not require a lexicon, it also supports Out-of-
    Vocabulary words. The main contributions of this paper are the interaction
    technique and the evaluation of this input method.

    Overall, the paper is well written and easy to follow. However, I think the
    motivation for supporting Out-of-Vocabulary words needs to be improved. Is not
    supporting OOV words actually a problem? Here the authors should look for existing
    works that show that this is or could be a potential problem. Otherwise, the
    motivation for the technique is, in my opinion, not very strong.

    The user studies and the design of the DuSK technique seem very solid. The
    explanations are mostly clear and are reasonable. I would be interested if the
    authors also measured the length of thumbs? Maybe this could influence the
    results, especially in a between-group study setup with two device sizes.

    In my opinion, the use cases for this interaction technique a very vague the
    authors mention several times that it could be used in combination with a SmartTV
    or in VR. However, they do not provide a lot of details about this. So, for
    example, in which VR context would this system be used? Typically in VR, users
    already have the VR controllers in their hands. In which situation should they
    switch to another device that the users have to hold in both hands for creating
    touch input. Here the authors should provide more details about possible use
    cases.

    Overall, I think the studies are well-executed, and the design process provides a
    lot of insides. However, the authors need to improve the motivation and the
    possible use cases of the proposed technique. I am looking forward to a strong
    rebuttal.

  Rebuttal response

    (blank)

----------------------------------------------------------------

reviewer 1 review
score 3/5

  Expertise

    Knowledgeable

  Recommendation

    Neutral: I am unable to argue for accepting or rejecting this paper; 3.0

  Review

    ===== Significance of the paper's contribution =====
    This paper presents an interesting indirect text entry technique achieved by
    bimanual drag-based input. The approach that the authors used is reasonable, which
    also supports OOV words. The results of the studies are rich and convincing. Other
    researchers can easily reproduce the technique by the authors' code.

    ===== Originality of the work =====
    The interactive method is new: indirect, bimanual, drag from fixed start points,
    not rely on a lexicon.

    ===== Validity of the work presented =====
    Good.

    ===== Presentation clarity =====
    Good.

    ===== Relevant previous work =====
    [1] Zhican Yang, Chun Yu, Xin Yi, and Yuanchun Shi. 2019. Investigating Gesture
    Typing for Indirect Touch. Proc. ACM Interact. Mob. Wearable Ubiquitous Technol.
    3, 3, Article 117. https://doi.org/10.1145/3351275.
    [2] Andrew Fowler，Kurt Partridge，Ciprian Chelba，Xiaojun Bi，Shumin Zhai. 2015.
    Effects of Language Modeling and its Personalization on Touchscreen Typing
    Performance. In CHI Conference on Human Factors in Computing Systems Proceedings
    (CHI 2015). https://dl.acm.org/doi/10.1145/2702123.2702503.
    [3] Yiqin Lu, Chun Yu, Shuyi Fan, Xiaojun Bi, Yuanchun Shi. 2019. Typing on Split
    Keyboards with Peripheral Vision. In CHI Conference on Human Factors in Computing
    Systems Proceedings (CHI 2019). https://doi.org/10.1145/3290605.3300430.

    ===== Major concerns =====
    1. Cursor visual feedback. In the final technique, the users can see two cursors
    to help point at the target key. But in Study 1, there is no such feedback. This
    inconsistency makes Study 1 provide little contribution to latter design and
    studies.
    In my opinion, indirect touch inputs with and without cursor feedback are totally
    different. Indirect touch input with cursor feedback requires the user to adapt
    his/her motor skill to the UI. It is more like "drag", which consists of moving
    and clutching. On the other hand, indirect touch without cursor feedback is based
    on the user's proprioception, like many gestural inputs.
    So, L-shape and V-shape strokes are actually gestural inputs, and they are
    certainly abandoned in later design/technique. Also, the results of Task 2 in
    Study 1 - the mapping doesn't work.
    The authors should think carefully about which parts in Study 1 are relevant to
    design/technique and reorganize Study 1 to provide meaningful insights that may
    benefit the final design/technique.

    2. The rationality of two start points 'D' and 'K'. The authors pay little
    attention to the choice of the start points of the left and right thumbs. What
    about 'S' and 'K'? Or 'D' and 'J'? Maybe 'D' and 'K' are the best, but readers
    need convincing results. The authors should provide at least a simulation to show
    why this choice is reasonable. Like the previous work [1], it also explores
    indirect text inputs tasks and concludes 'G' is the best start point with some
    quantitative data.

    3. Novice and expert transition. Despite the high learning cost of DuSK, the
    exploration of novice-expert transition will be interesting. However, the paper
    disappoints me. First, the results don't reflect "transition", which should start
    from the novice stage. This paper only shows data of two experts after two-hour
    training. What about the speed and accuracy of the first two hours? By the way, I
    think the first two hours are de facto "transition" (learning). Second, I think
    authors are not appropriate to be the evaluated experts. Authors know all the
    tricks of the technique in the beginning, which much affects the learning curve.

    4. OOV. The authors claim their technique supports OOV words strongly, and I also
    agree it is the highlight of this technique. However, in Study 2, the authors
    evaluated the technique in MacKenzie et al.'s phrase set. As I know, there are
    very few OOV words in this set excluding the top 50000 words in American National
    Corpus. What's the OOV rate of this phrase set [2,3]? How auto-correction
    influences the behavior of typing OOV words [2,3] (i.e., false auto-correction
    problem)?

    ===== General comments =====
    I really like this technique, although it's not easy to type fast. I definitely
    agree that this technique should be published in CHI conference. However, the
    major concerns above prevent me from accepting the paper in the current stage. I
    stand neutral, and I welcome the authors to address my concerns to raise my score.

  Rebuttal response

    (blank)

----------------------------------------------------------------

reviewer 2 review
score 2.5/5

  Expertise

    Knowledgeable

  Recommendation

    . . . Between possibly reject and neutral; 2.5

  Review

    This paper presents the design and evaluation of a dual-hand text entry system for
    touchpad-based indirect input. It combines tapping and strokes to support fast
    text input and inputting out-of-vocabulary words. Novice users could reach a
    typing speed of 13 WPM after short training.

    For indirect text input, previous works usually rely on the lexicon to reduce the
    input noise and infer the intended word. This paper took a different approach: the
    users could use a single unambiguous and location-independent action (either a tap
    or a single directional stroke) to enter any character on the keyboard. This
    approach also enables the input of OOV word, which the lexicon-based methods could
    not achieve. The proposed solution is new, and the method described in the paper
    is valid.

    Overall I find this paper very well presented and easy to follow. However, I do
    have some concerns regarding the system that require some clarification from the
    authors.

    - Experiment design of Study 1:
    Study 1 explored various actions that can support letter-by-letter text input;
    however, I don't fully understand how the findings were later used in the design
    of DuSK. For example, in task 1, the touchpad is divided into 9 equal-sized cells.
    How would this help the readers estimate the tap accuracy on a full keyboard with
    much smaller keys? Since taps were the fastest and the most accurate action, why
    were they only used to enter the two keys at the starting location ("D" and "K")
    but not more? The time measurement results are not surprising, considering that
    the stroke length is different for single directional, L-shaped, and V-shaped
    strokes. It might be more interesting to compare the input speed in mm/s. In task
    2, were the participants required to only use single-directional strokes? If not,
    how were the angle and length computed for L-shape or V-shaped strokes?

    - Evaluation:
    An important contribution of this work is that it enabled entering OOV words,
    "such as usernames, passwords, website addresses, proper names." However, this was
    not properly evaluated. In study 2, the participants transcribed sentences from
    the MacKenzie and Soukoreff phrase set, which only contains dictionary words. I
    would suggest the authors include some form of evaluation to highlight this
    benefit since the input speed on dictionary words is much lower than other
    lexicon-based text entry systems.

    Considering the learning curve of the proposed method, it might also be worth it
    if the participants were given a longer training session. The authors also showed
    that expert users (authors A and B) could reach as high as 33 WPM with the
    proposed text entry method. How long have the expert users used this system to
    achieve such a performance?

  Rebuttal response

    (blank)

----------------------------------------------------------------


==> tex/IMWUT_reviews.tex <==
Reviews for IMWUT 2021 (February 2021 round) submission 1758:



----------------------------------------------------------------

1AE review

  1AE's recommendation to Editors

    Major revisions (enumerated in a subsequent field) are required for this to be publishable

  Impact

    Low impact

  1AE's meta-review

    Overall, reviews state that this is a well-motivated work (2AE, R4) that presents an interesting idea (R3) to a challenging problem (2AE). The related work is mostly comprehensive (2AE, R4), with exception of a few missing references (R4). The paper follows best practices in text-entry interaction design and empirically evaluates their proposed design (2AE, R3), though the empirical study does not
    directly compare against another text-entry technique.

    However, the reviews point to a number of items that must be addressed prior to publication.

    The paper overclaims the performance of the proposed technique (2AE, R4). The paper provides anecdotal evidence about possible expert performance collected from 2 authors (2AE, R4) that far exceeds otherwise mediocre performance from the empirical study (R3). Any such claims should be removed in major revisions (R4). Note however that an upper bound on expert performance could still be useful to compare against other existing techniques (2AE). One way to compute such a bound is using a model of expert text entry similar to [1]; though considering that the error rate could be high with the proposed interaction and that DuSK still uses a form of automated correction, it may also be important to consider or at least discuss effects of errors on the modeled upper bound expert text-entry speed (please see references for more details about relevant models).

    All reviews ask for clarification about study design and analysis (2AE, R3, R4). The exact description of the study design is unclear (R4), which makes it difficult to ensure DuSK can be compared to techniques in [21]. Also, comparison with the other techniques is not appropriate because each of those studies was different in many ways (task, participants, duration, etc.). Although it is true that some state-of-the-art baselines may struggle with out-of-vocabulary words, it is not clear how represented such words are in a word corpus, and if handling of out-of-vocabulary words justify the low performance of DuSK in all other situations (2AE, R3). Furthermore, the empirical study uses an existing phrase set [23] which does not contain many (if any) out-of-vocabulary words. Thus, the revisions should make it clear when comparison with performance of other text- entry techniques collected in existing empirical studies is appropriate and better quantify the effects of out-of-vocabulary words on typist performance.

    The reviews ask for clarification about design decisions that informed the design of DuSK (2AE, R4). Major revisions should make it clear what role insights from early interactions play in the final design (2AE). Major revisions should also justify focus on performance (speed, accuracy) compared to other important considerations (ergonomics, learnability) (R4).

    Reviews ask about novelty to DuSK (R3, R4). The revision should call out the knowledge the work generates past what the reader can already learn about eyes-free text entry from [1] and [21].

    In summary, this work could generate new knowledge about eye-free text entry on mobile touchscreen devices that could be of interest to the IMWUT community. However, the paper must address items above prior to publication. Thus, I look forward to a revised version.


    REFERENCES
    @inproceedings{DBLP:conf/chi/BanovicRSDM17,
      author    = {Nikola Banovic and
                   Varun Rao and
                   Abinaya Saravanan and
                   Anind K. Dey and
                   Jennifer Mankoff},
      editor    = {Gloria Mark and
                   Susan R. Fussell and
                   Cliff Lampe and
                   m. c. schraefel and
                   Juan Pablo Hourcade and
                   Caroline Appert and
                   Daniel Wigdor},
      title     = {Quantifying Aversion to Costly Typing Errors in Expert Mobile Text
                   Entry},
      booktitle = {Proceedings of the 2017 {CHI} Conference on Human Factors in
    Computing
                   Systems, Denver, CO, USA, May 06-11, 2017},
      pages     = {4229--4241},
      publisher = {{ACM}},
      year      = {2017},
      url       = {https://doi.org/10.1145/3025453.3025695},
      doi       = {10.1145/3025453.3025695},
      timestamp = {Sun, 25 Oct 2020 22:41:01 +0100},
      biburl    = {https://dblp.org/rec/conf/chi/BanovicRSDM17.bib},
      bibsource = {dblp computer science bibliography, https://dblp.org}
    }

    @inproceedings{DBLP:conf/mhci/BanovicSHDM19,
      author    = {Nikola Banovic and
                   Ticha Sethapakdi and
                   Yasasvi Hari and
                   Anind K. Dey and
                   Jennifer Mankoff},
      title     = {The Limits of Expert Text Entry Speed on Mobile Keyboards with
    Autocorrect},
      booktitle = {Proceedings of the 21st International Conference on Human-Computer
                   Interaction with Mobile Devices and Services, MobileHCI 2019,
    Taipei,
                   Taiwan, October 1-4, 2019},
      pages     = {15:1--15:12},
      publisher = {{ACM}},
      year      = {2019},
      url       = {https://doi.org/10.1145/3338286.3340126},
      doi       = {10.1145/3338286.3340126},
      timestamp = {Sun, 25 Oct 2020 23:06:37 +0100},
      biburl    = {https://dblp.org/rec/conf/mhci/BanovicSHDM19.bib},
      bibsource = {dblp computer science bibliography, https://dblp.org}
    }

  1AE's meta-review: Major / minor revisions

    Major revisions:
    -   Add missing references.
    -   Remove overclaims about expert performance with DuSK.
    -   Consider adding a model to compute expert performance with DuSK and compare it with a baseline.
    -   Clarify study design.
    -   Avoid comparison with empirical studies that used a different study protocol and those where participant population differs from participants in the empirical study reported in the paper.
    -   Quantify effects of out-of-vocabulary words and justify low walk-up-and-use performance with DuSK.
    -   Discuss novelty of DuSK compared to existing work.

----------------------------------------------------------------

2AE review

  Contribution to IMWUT

    This paper investigates bimanual eyes-free text entry using touch screen devices, specifically addressing Out-Of-Lexicon words. They present a study on user generation of eyes free gestures on a touchscreen, looking at single strokes, compound strokes, and taps. Using this study results, as well as an iterative design process, they created a method for bimanual stroke input on a virtual kepays, DuSK. They conduct a evaluation of the text entry technique and compare it to a cursor based method, commonly used on smart tvs, and found their performed better.

  Impact

    Low impact

  Review

    Overall, I found this paper to be well motivated, conducted, and written, though there are a number of grammatical issues to be addressed. The problem of eyes-free text entry remains a challenge, in a number of contextual settings, which the authors describe. Here they focus on eyes-free text entry for non-collocated displays, such as a smart tv. The authors do a good job of providing a survey of existing techniques, although I am not an expert in this area.

    However, I have a number of concerns with the paper and their approach. 1) Overclaims, 2) a reasonable baseline comparison, 3) how we learn from the iterative design. These issues, which I detail below, reduce the contribution of the paper.

    Overclaiming - 
        Personally, I felt the paper overclaims on how well the system performs.
    They often use the expert typing speed from the authors to motivate the benefits of the system, however, they do not report any ceilings for other competitive designs. Without this information about other expert use ceilings it is hard to evaluate. Additionally, the walk up and use improvement compared to the chosen baseline, is a substantial improvement (25\%), but I believe this is a strawman
    comparison. More about the control condition below:

    Reasonable Baseline Comparison

    Overall, I found the comparison to the cursor based soft text entry to be not an ideal comparison. While it is true this technique is used widely, it is not anywhere near the state of the art. For example, an alternative might be eyes-free gesture writing with a cursor and the second hand used to engage/disengage the stroke. I was unconvinced that the selected technique was a reasonable baseline.

    What do we learn from the iterative design?

    While I am a proponent of iterative design, I found it hard from that section to draw too many insights. More details are needed as well as potentially more participants to make any meaningful claims.


    Additional comments:


    Study 1:
    More detail is needed on how the gesture set was selected.

    4.1.2 -> Touchpad size - it was unclear what Small or Big was. I assume the 5.9vs 6.3 inch displays? More detail should be included about what that variable is and why these two sizes were selected.

    4.1.3 -> Why is the touchpad divided in to 9 cells, what is the reasoning or motivation.

  Recommendation(s) to 1AE

    Major revisions (enumerated in a subsequent field) are required for this to be publishable, Reject

  Major / minor revisions (recommendation to 1AE)

    See above

  Confidence

    Somewhat confident - I have passing knowledge

----------------------------------------------------------------

Reviewer 3 review

  Contribution to IMWUT

    Please refer to my review.

  Impact

    Low impact

  Review

    I reviewed this paper in another conference last year.  At the time the paper was rejected. Although the authors made some minor changes, the main issues remain unaddressed and it would be hard for me to argue for acceptance.

    Below is my review. Some content is similar to what I provided last year, because the same issues remain unaddressed.

    This paper presents a two-handed text entry method called DuSK. It maps the finger strokes on two sides of a Qwerty keyboard to letters, and uses a statistical decoding method to decode the input.  DuSK was designed following an iterative design procedure. The authors first carried out studies to understand users’ ability of executing strokes, and leveraged the understanding to guide the keyboard design. Users studies were conducted to compare DuSK with a cursor based text entry method.

    This paper presents an interesting idea, leveraging two-handed finger strokes for text entry. The authors did a reasonably good job to execute the project and formally evaluate it. However, overall I am lukewarm and it is hard for me to argue for acceptance, because of the following reasons.

    The main issue is that  the evaluation shows the performance of DuSK is mediocre, compared with many existing text entry methods.  The input speed of DuSK is below 15 WPM, more than 25\% slower than the similar text method for smart TV such as blind type [21] and i’s Free [45]. Additionally, the study has a major flaw: it omits a very important and natural baseline: two finger typing on a regular
    virtual keyboard displayed on the TV. Such a method would have a similar UI design with DuSK, require two-handed input, and support out-of-vocabulary words input (by displaying the literal string suggestion on the suggestion bar). It is an apparent baseline and would help us assess the efficacy of DuSK. The current baseline in the paper, the cursor-based method has been shown a very poor baseline [21] and was originally designed for button based text entry. Improving text entry performance over such a method would be a very low bar.  Because of the nature of the work -- applying an existing technique (stroke-based method for text entry) to solve a problem in a new domain, it is necessary to have evidence showing that such a technique is worth adopting. Unfortunately, I do not see convincing evidence in the evaluation.

    The authors explained that BindType cannot support OOV words so that it was excluded as a baseline. It was a false statement.  The BlindType [21] method can actually support OOV input: the sequence of typed letters (i.e., the string before
    being fed into the statical decoder) can be displayed as an option on the suggestion bar. This is actually how the current touchscreen keyboard on smartphones works: you can always get the sequence of typed letters, which sometimes are OOV words, as one of the suggestions in the suggestion bar.


    Second, the paper lacks novelty. DuSK boils down to applying the two-handed finger strokes for text entry. Marking menu has been a classical research topic in HCI, and the two-handed marking menu has been thoroughly studied in literature [15]. Using finger strokes for text entry has also been investigated before (e.g., SwipeBoard [5]). The only technical contribution of DuSK, in my opinion, is about applying an existing technique (two-handed marking menu strokes) to a new domain (text entry).  It is common in research that researchers apply a known technique to solve a problem in another domain. However, the value of such work will largely depend on whether the technique is really effective for the problem. In that regard, the results are disappointing, as explained above.

    Overall, my recommendation of the paper remains the same as last time I reviewed it. It is disappointing that the authors did not revise the paper according to the reviewers’ comments (e.g., having an adequate baseline in the experiments).

  Recommendation(s) to 1AE

    Reject

  Major / minor revisions (recommendation to 1AE)

    (blank)

  Confidence

    Highly confident - I consider myself an expert in the area

----------------------------------------------------------------

Reviewer 4 review

  Contribution to IMWUT

    DUSK is an indirect text entry method for touchpads that supports out-of-vocabulary words. The form factor and design could fit smart TVs and HMDs, which still lack efficient text entry methods. Intelligent text entry methods suggested for these, on the other hand, suffer from OOVs. A benefit of the proposed method is that it is stroking-based, which  allows retaining gaze on display and not on
    keyboard.

  Impact

    Medium impact

  Review

    The paper starts by providing a motivation for the problem and a relatively comprehensive overview of existing literature. With the exception of two references, I found it adequate. Buschek (2014, IUI) and Schoenleben (2013, MobileHCI) have presented probabilistic methods for tapping-based entry on mobile surfaces [bibtexs below].

    The paper then presents design goals, which I think was comprehensive, however with the exception that learnability and ergonomics are missing, which are obviously important. Also, I would have liked to see a bit more discussion on how to operationalize these metrics. The only one that is properly operationalized is efficiency. What is known about the others in this class of methods?

    Then, a study is presented to collect gestures for letter-by-letter entry. Then the design of the system is evolved over several iterations. It has many similarities when compared to BlindType [21]. The authors could expand discussion of novelty over [21] in Introduction.

    The reporting of empirical methods should be improved. The paper refers to Lu et al [21] on how the evaluation study was done. I think for self-sufficiency the main aspects of the study should be reproduced in this paper. For example, Lu et al. describe  multiple studies: which one was the one that was followed?
    
    My main concern with this paper is that it alludes to high WPMs in Abstract, but these observations are anecdotal. The authors report their own performance as an estimate of 'performance ceiling'. These values are also reported in Abstract ("with training"), giving the reader an illusion that this was observed in the study. This is borderlining dishonesty and would be embarrassing for the field and
    the journal to publish this like this. These results are not from representative users, and training is not properly described, at all. The data is entirely anecdotal. That some earlier paper has done this does not make this a good estimate of achievable rates. I recommend removing this part.


    @inproceedings{buschek2014improving,
      title={Improving accuracy in back-of-device multitouch typing: a clustering-
    based approach to keyboard updating},
      author={Buschek, Daniel and Schoenleben, Oliver and Oulasvirta, Antti},
      booktitle={Proceedings of the 19th international conference on Intelligent User
    Interfaces},
      pages={57--66},
      year={2014}
    }

    @inproceedings{schoenleben2013sandwich,
      title={Sandwich keyboard: Fast ten-finger typing on a mobile device with
    adaptive touch sensing on the back side},
      author={Schoenleben, Oliver and Oulasvirta, Antti},
      booktitle={Proceedings of the 15th international conference on Human-computer
    interaction with mobile devices and services},
      pages={175--178},
      year={2013}
    }

  Recommendation(s) to 1AE

    Major revisions (enumerated in a subsequent field) are required for this to be
    publishable

  Major / minor revisions (recommendation to 1AE)

    Remove the part anecdotal part (see review)

    Improve reporting of empirical methods

    Improve design goals and literature

  Confidence

    Highly confident - I consider myself an expert in the area


==> tex/changes.tex <==
Many thanks for the detailed and helpful comments. We have modified the paper to accommodate the reviewers’ comments as follows. New content highlighted in blue in the paper, and deleted comments indicated in red.

\section{Missing references (1AE, R4)}
\begin{itemize}
    \item We incorporated the missing references into the related work
\end{itemize}


\section{Remove Overclaims about Expert Performance (1AE, 2AE, R3, R4)}
\begin{itemize}
    \item We removed all claims of expert performance using the results of the two authors.
    \item We removed the section `Performance Deconstruction' which presented the results of the two authors.
    \item We added a section `Predicting Expert Performance' in which we propose a model to predict the peak performance that can be obtained with \name and add the results of the 2 authors as a sanity check.
\end{itemize}

\section{Clarify Study Design (1AE, R4)}
\begin{itemize}
    \item We clarified the protocol followed in Study 2 and added details about which study we are referring to.
\end{itemize}

\section{Avoid comparison with empirical studies that used a different protocol}
\begin{itemize}
    \item We removed comparisons with techniques with different protocols in Study 2's results section
\end{itemize}

\section{Clarify insights from early interactions play in final design (1AE, 2AE)}
\begin{itemize}
\item We separated early iterations from the final design in two distinct sections
\item We added a subsection summarising all insights drawn from the iterative design study which influenced the design of the final iteration.
\end{itemize}

\section{Justify low walk-up-and-use performance with \name (1AE, R3)}
\begin{itemize}
    \item We clarified use-cases for \name and justified its use in light of the results in the Discussion.
\end{itemize}

\section{Discuss novelty of DuSK compared to existing work (1AE, R3, R4)}
\begin{itemize}
    \item We clarified our work's contribution and novelty in Introduction 
    \item We added details on how \name differs in Related Work
\end{itemize}

\section{Clarify how to operationalize design goals (R4)}
\begin{itemize}
    \item We modified the description of the design goals to include concrete ways of operationalizing them.
    \item We added details and references to the design goals while presenting \name's design and the results of the experiments.
\end{itemize}

\section{Quantify effects of out-of-vocabulary words (1AE)}
1AE is concerned that the empirical study does not properly assess \name's performance with OOV words, i.e., ``\textit{The empirical study uses an existing phrase set [23] which does not contain many (if any) out-of-vocabulary words}''

We agree that MacKenzie and Soukoreff's phrase set~\cite{10.1145/765891.765971} does not contain many out-of-vocabulary words. We primarily tested \name using this dataset as to allow for a comparison with \cite{blindtype}. As a result, we performed a second experiment (Study 3) in which we evaluate \name on a phrase set of OOV words~\cite{velocitwatch}. The results showed that the performance obtained on this new phrase set of OOV words is not statistically different from the ones obtained in Study 2, suggesting that \name can enter both in-vocabulary and out-of-vocabulary with similar performances (in terms of speed and accuracy).

\begin{itemize}
    \item We clarified the goal and motivation of Study 3.
\end{itemize}


\section{Justify focus on performance (speed \& accuracy) (1AE, R4)}
R4 asks why we did not address ergonomics and learnability. While we did not mention learnability and ergonomics as design goals, we did consider these aspects while designing \name: (1) Ergonomics is addressed implicitly in study 1 by measuring and contrasting the time of gesture variants. (2) Issues of learnability are also addressed via the multi-session study in study 2 and in the pilot study (i.e. we preserve qwerty layout to foster learnability).

\begin{itemize}
    \item We added justifications regarding our choice of design goals
\end{itemize}

\section{Reasonable Baseline Comparison (R3, 2AE)}
\subsection{BlindType (R3)}
R3 is concerned that BlindType may support Out-of-Vocabulary eyes-free input, i.e. ``\textit{The BlindType [21] method can actually support OOV input: the sequence of typed letters (i.e., the string before being fed into the statical decoder) can be displayed as an option on the suggestion bar.}''. This claim seems at odds with the information contained in the paper by Zhu et al.~\cite{blindtype}, so we contacted the authors of BlindType. The first author's email response (emphasis is the first author's, i.e. this is the verbatim email response) is as follows: 

\textit{``BlindType does NOT support OOV words. The noise of touch input makes it hard to interpret individual keystrokes.
To support precise character-level input, BlindType should show the visual feedback of a touch position on the screen and allow the user to adjust the position. The input speed will definitely decrease.
Also, BlindType can be supplemented with other eyes-free character-based text input methods (e.g., hand-writing) to work for OOV words.''}

While we believe that adapting BlindType to allow OOV is an interesting research direction, it has never been explored, is non-trivial, and the feasibility is uncertain. Designing and evaluating such a method is therefore out of the scope of our paper. Thus, we believe that the cursor-based method is a more reasonable baseline.

\begin{itemize}
    \item We clarified the reasons making BlindType unable to enter OOV words and acknowledge that a modification could allow the technique to support OOV words but the feasibility is uncertain in Related Work.
\end{itemize}

\subsection{Two finger typing on a regular virtual keyboard (R3)}
R3 suggests another technique that we could compare \name against: ``\textit{Additionally, the study has a major flaw: it omits a very important and natural baseline: two finger typing on a regular virtual keyboard displayed on the TV.}

Lu et al. showed that users are inaccurate when tap-typing eyes-free~\cite{blindtype} and that intelligent disambiguation mechanisms -- with a language model -- are necessary. Thus, we did not consider this baseline.
%Such a technique would be similar to BlindType but two-handed. As such, it is unclear how can the technique be implemented to support OOV words. Lu et al. demonstrated that users are not able to accurately tap-type eyes-free~\cite{blindtype} and that intelligent disambiguation mechanisms are necessary to decode their input.


\subsection{Eyes-free gesture writing (2AE)}
2AE suggests that the evaluation might have compared \name with other techniques, i.e.,``\textit{I found the comparison to the cursor based soft text entry to be not an ideal comparison. [...] an alternative might be eyes-free gesture writing with a cursor and the second hand used to engage/disengage the stroke.}''

Such a technique would leverage the gesture writing algorithm~\cite{gesture_typing} and thus forbid Out-of-Vocabulary words. The entry of OOV words being one of the motivation that drove the design of \name, we believe that such a comparison would be unfair. To the best of our knowledge, the cursor based method is the only method offering capabilities similar to \name and thus is a reasonable baseline.

\begin{itemize}
    \item We clarified that gesture writing-based approach do not allow OOV words in Related Work.
\end{itemize}

\section{Other (2AE)}
\begin{itemize}
    \item We added details on how the gesture set for Study 1 was selected
    \item We clarified the variable "Touchpad size" in Study 1 and added justification
    \item We added a justification for dividing the touchpad into 9 cells.
\end{itemize}

\newpage

==> tex/expert_study.tex <==

\section{Performance deconstruction} \label{deconstruct_perf}
The previous sections showed that \name outperforms the cursor-based text entry method with and without training. Our results suggest that participants are still improving after 40 minutes. In this section, we deconstruct participants' performance with \name in order to understand \textit{how} users improve, and \textit{what} causes their performance. Similar to Kristensson and Zhai~\cite{gesture_typing}, we estimate \name's performance ceiling (i.e. how fast a user could eventually enter text) by measuring the performances achieved by two authors after extensive training. \textit{Author A} and \textit{Author B} trained with \name until they felt confident with the technique (approximately 2 hours). Both authors then did the study following exactly the same protocol as Study 2. Therefore, they both had to transcribe 56 sentences, 40 without autocorrect nor word completion. In the rest of the section, we compare the performance of Study 2's participants (referred to as \textit{Novices}) against those of two authors (referred to as \textit{Experts}).
%we compare the performances obtained by participants in Study 2 (referred to as \textit{novice users}) to those of 2 \textit{expert users}. Our motivation is twofold: first, we wish to evaluate how fast one can type using \name given significant experience with its use; second, we want to investigate how one transitions from novice to expert.  Our method for this assessment, leveraging two expert users, echoes the assessment of Kristensson and Zhai \cite{gesture_typing}.

%\footnote{An alternative method to complete this study would involve a longitudinal study with users. Because the current worldwide health environment precludes contact with users in controlled environments, we present this analysis to complement our Study 2's single-session summative assessment.}.

%Therefore, we investigate the performances of expert users with \name (expert users referring to users with extensive training).
%Previous work used several ways to evaluate expert performances, either by asking a small number of participants to train for longer, using an equation to approximate the evolution of WPM~\cite{perkinput} or entering the same sentence multiple times and presenting the best results~\cite{gesture_typing}. We use a mix of these techniques to estimate experts users' speed and accuracy.

\subsection{Measurements}
Essentially, the time to enter a character with \name is divided in two parts: first, locating the character and deciding which thumb to use (\textit{Reaction time}); second, stroking towards this character (\textit{Stroke time}). We measure the \textit{reaction time} as the time between the end of a stroke, and the beginning of a new stroke. Similarly, we measure the \textit{stroke time} as the time between the touch down event that started the stroke, and the corresponding touch up event.
We also measure accuracy, specifically the corrected error rate which corresponds to how frequently a user used `Backspace' to correct a mistake and could therefore cause slower text entry.

%\begin{figure}[t]
%	\centering
%	\includegraphics[width=1\textwidth]{figures/results/deconstruct_results_1col.pdf}
%	\caption{Means and standard deviation of the reaction time, stroke time, and corrected error rate of both novice and expert users by block. Autocorrect and suggestions was added to the last two blocks.}
%	\label{fig:results_breakdown}
%\end{figure}

{\centering
     \includegraphics[width=1\textwidth]{figures/results/deconstruct_results_1col.pdf}
      \captionof{figure}{Means and standard deviation of the reaction time, stroke time, and corrected error rate of both novice and expert users by block. Autocorrect and suggestions was added to the last two blocks.}
	\label{fig:results_breakdown}
      \par}
      

\subsection{Results and Discussion}

Using \name character-by-character without predictions, Author A average speed was 29.9 WPM (\std{4.3}) for an uncorrected error rate of 1\% (\std{2.3}). Author B average speed was 23.6~WPM (\std{2.9}) for an uncorrected error rate of 2.6\% (\std{3}).
The results were slightly different with the introduction of autocorrection and word completion. Author A achieved 33.2~WPM (\std{7.6}) and Author B achieved 22.9~WPM (\std{6}) for an uncorrected error rate of 0.8\% (\std{1.7}) and 1.14\% (\std{2.6}) respectively.
Below we summarise the results of our analysis. p-values are calculated using Welch's t-test or ANOVA. The breakdown of the results can be visualized in Figure~\ref{fig:results_breakdown}. We analysed the last two blocks with predictive algorithms separately.
% Because the error rate between novice and experts is not significantly different, we measure performance solely based on wpm.



\textbf{Reaction time.} Experts had significantly lower reaction times than novices ({\small 145ms vs 446ms, p<.001}). Interestingly, novices' reaction time steadily decreased with training. Granted that the decrease rate stays the same, a linear regression predicts that novices would reach experts' reaction time on the 11th block (about an hour).

We also measured the reaction time when switching hands (e.g. the reaction time between stroke A and stroke B, where stroke A was done with the left thumb, and stroke B with the right thumb) compared to using the same hand. Novices had significantly faster reaction times when alternating hands as opposed to using the same hand ({\small \mean{439ms} vs \mean{453ms}, p=.017}) and the difference was even more pronounced with expert users ({\small 116ms vs 172ms, p<.001}) suggesting that \name benefits from being two-handed.

\textbf{Stroke time.} Experts had significantly lower stroke times than novice users ({\small 348ms vs 657ms, p<.001}). We found a significant effect of block on stroke time for novice users (\anova{2}{20}{4.66}{.025}) but only between the first block and any other block. It is therefore unclear how and when users transition to experts' stroke times and may simply be caused by users becoming more confident with the technique (similar to the drop in stroke time between first and second block).


\textbf{Accuracy.} Both expert and novice users left a similar number of uncorrected errors ({\small 1.7\% vs 1.2\%, p=.19}). However, experts corrected significantly fewer mistakes ({\small 4.15\% vs 6.5\%, p=.004}) suggesting that accuracy improves with training despite faster strokes and reaction times, contributing to increased expert performance.

\textbf{Autocorrect and word completion.} Interestingly, introducing suggestions and autocorrect induced a significant increase of reaction time for both experts ({\small 145ms vs 279ms, p<.001}) and novice users ({\small 446ms vs 636ms, p<.001}), possibly caused by the cost of attending to suggestions~\cite{benefit_suggestions}.
Additionally, experts stroked faster with predictive algorithms ({\small 275ms vs 348ms, p<.001}) but not novice users ({\small p=0.28}). When autocorrect was available, experts used it to correct 4\% of words (novices: 1.7\%) and auto-completed 67.4\% of words (novices: 70.6\%), suggesting that relying on predictions allowed experts to stroke faster.

Finally, despite higher reaction times, both experts and novices improved entry rate (respectively 27~WPM and 13.1~WPM) indicating that the benefit of predictive algorithms is higher than their cost~\cite{benefit_suggestions}.

==> tex/rebuttal.tex <==
Thank you for the detailed reviews! We are pleased reviewers found the paper "very well presented and easy to follow" (R2), the studies "well-executed" (R3), the results "rich and convincing" (R1), and that "this technique should be published in CHI" (R1).

Reviewers also expressed concerns; we detail below how we propose to address them in a minor revision. Order follows R4's list.

# Use cases (R3)
There is significant work leveraging attendant mobile devices for interacting with external displays/VR: 
- Alongside [21, 43], the Pebbles project at CMU (personal devices as universal remote control), e-learning systems like Kahoot, and gaming platforms like AirConsole all propose using smartTVs plus personal devices in concert. Leveraging the "at-hand" device seems convenient. 
- Smartphone-tethered systems such as Huawei VR Glass have an attendant smartphone which can be leveraged for input, and so is a natural target for DuSK.
- Using smartphones as controllers for HMDs is fairly common (e.g. Oculus Go) and systems such as Google Cardboard could be extended to leverage two connected devices for input.
Despite all of the above, R3 makes a good point that, in systems with dedicated controllers, switching to another device is inconvenient. However, we note that while we evaluated DuSK using a smartphone with the screen turned off, DuSK can also leverage the touchpads already present on SmartTVs and VR controllers (e.g. AppleTV remote, Playstation controller) or bi-manual touchpads (e.g. HTC Vive controllers) in which case users do not need to switch devices.
> ACTION: We will highlight the above points more clearly and add concrete use cases in Intro.

# Motivation for OOV (R3)
We believe that OOV words are important to consider and that a significant weakness of [21, 43] is that these systems completely ignore OOV, because: 
- OOVs are frequent when messaging and on social media (10.1145/2414425.2414430). 
- With SmartTVs and VR, OOVs are required for information such as passwords, email addresses and names (e.g. in-app purchase in VR 10.1145/3334480.3382827) but can also appear in movie titles, in-game chats, etc.
> ACTION: We will add motivating examples in Intro to highlight the importance of deterministic text input to handle OOVs and other downsides of false auto-correction and collisions [DOI:10.1145/2702123.2702503, 10.1145/3338286.3340126, 26, 30].

# Evaluating OOV (R1, R2) 
We acknowledge that our testing evaluated *deterministic text input*, i.e. text input that is generated without the use of a dictionary. Deterministic text input without a dictionary essentially reduces the vocabulary to size 0 such that all input is "OOV". It is important to remember that OOV is not equivalent to unpracticed input for a user. For example, personal telephone numbers, usernames, email addresses, or passwords are all OOV, but not unpracticed.
We used the phrase set from [21, 43] for fair comparison, and study 2 showed that DuSK outperformed the only other method supporting *deterministic text input*.
> ACTION: We will be very clear in text that we evaluate *deterministic text input*, or *text input without auto-correct*. In implications, we will note that DuSK's ability to support deterministic text input allows DuSK to support OOVs (unlike [21, 43]).
> INFORMATION: To answer your specific questions, a post analysis revealed that 7.5\% of sentences entered during study 2 contained at least one OOV word (i.e. a word not among 50,000 most common). A t-test did not find a significant difference between the WPM/Error rate of sentences with/without OOV (p>.05)

# Visual feedback/Contribution of Study 1 (R1, R2)
We agree that visual feedback might impact results. In fact, we experimented with cursor visual feedback with DuSK's final iteration, following a participant’s suggestion. Early iterations, including the ones experimenting with V/L-Shapes did not use such feedback (see Fig. 6/7 vs 8) therefore Study 1’s results do apply.
Study 1 was exploratory and its results were combined with informal studies to guide the design of DuSK.
As a result, DuSK uses a subset of the actions tested during Study 1:
- 8 taps (1-each for ‘D’ and ‘K’, Space, Enter, Backspace, and 3 for auto-correct suggestions)
- Single-Strokes of varying length.
- The transfer function computed from Task 2. 
We left the results for V/L-Strokes as we believe they are interesting and help understand our choices during the iterative design process.
> ACTION: Clarify our design choices with respect to Study 1 during the iterative design process and detail the use of visual feedback.

# ‘D’ and ‘K’ as start points (R1)
We acknowledge that details are missing about this choice. Because we use long/short strokes, there can be at most 2 keys mapped to a direction. ‘D’ is therefore the only possible choice on the left side. On the right side, both ‘J’, ‘K’ could work. We used ‘K’ as it reduces the number of keys in the bottom right corner, a direction that was shown to be difficult to stroke to with the right thumb [16].
> ACTION: Explain this choice and present ‘J’ as an alternative.

# Expert evaluation (R1, R2)
Similar to [18], we used two authors as "experts" for the sole purpose of measuring how fast a user could eventually write text with DuSK. We agree with R1 that authors have a different learning curve. As such, we did not report their learning curves. Instead, we compared the results of novices against "fully-trained" experts on the same study. We agree that the term “transition” is not the most appropriate here considering that the “transition” component has to be interpolated. Performance Ceiling is more appropriate.
> ACTION: Clean up terminology, discuss the use of authors as expert, and clearly state that authors' training time is not representative.

# Other
- R3: We did not measure participants' thumbs length.
- R2: mm/s is pertinent and we will also report it.
- R1: Thank you for the refs; we will incorporate in RW.
